FiT: Parameter Efficient Few-shot Transfer Learning for Personalized and Federated Image Classification

Modern deep learning systems are increasingly deployed in situations such as personalization and federated learning where it is necessary to support i) learning on small amounts of data, and ii) communication efficient distributed training protocols. In this work, we develop FiLM Transfer (FiT) which fulfills these requirements in the image classification setting by combining ideas from transfer learning (fixed pretrained backbones and fine-tuned FiLM adapter layers) and meta-learning (automatically configured Naive Bayes classifiers and episodic training) to yield parameter efficient models with superior classification accuracy at low-shot. The resulting parameter efficiency is key for enabling few-shot learning, inexpensive model updates for personalization, and communication efficient federated learning. We experiment with FiT on a wide range of downstream datasets and show that it achieves better classification accuracy than the leading Big Transfer (BiT) algorithm at low-shot and achieves state-of-the art accuracy on the challenging VTAB-1k benchmark, with fewer than 1% of the updateable parameters. Finally, we demonstrate the parameter efficiency and superior accuracy of FiT in distributed low-shot applications including model personalization and federated learning where model update size is an important performance metric.

==> tables/meta_trained_orbit_personalization.tex <==
\begin{table}[htbp]
    \vspace{-1em}
    \setlength\tabcolsep{1.2pt}
    \caption{ORBIT Personalization performance of \fit{}, meta-trained Simple CNAPs~\citep{bateni2020improved} and ProtoNets~\citep{snell2017prototypical}. Results are reported as the average accuracy (95\% confidence interval) over $85$ test tasks. Meta-trained model results are from \citep{bronskill2021memory}. Shared is the number of parameters shared among all users. Per User indicates the number of parameters stored for each user with $C$ classes. Average is the average number of individual user parameters for ORBIT dataset.   
    }
    \vspace{0.9em}
    \label{tab:meta_trained_orbit_results}
    \centering
    \scalebox{0.68}{
    \begin{tabular}{lcP{1.9cm}P{1.8cm}P{0.3cm}P{1.9cm}P{1.8cm}P{0.3cm}P{1.9cm}P{1.8cm}P{1.8cm}}
    \toprule
    && \multicolumn{2}{c}{\textbf{Clean Videos}} && \multicolumn{2}{c}{ \textbf{Clutter Videos}} && \multicolumn{3}{c}{\textbf{Parameters}}\\
    \cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-11}
    \textsc{\textbf{model}} && \textsc{\textbf{frame acc}} $\uparrow$ & \textsc{\textbf{video acc}} $\uparrow$ && \textsc{\textbf{frame acc}} $\uparrow$ & \textsc{\textbf{video acc}} $\uparrow$ && {\textbf{\textsc{shared}} $\downarrow$} & \textsc{\textbf{per user} $\downarrow$} & \textsc{\textbf{average} $\downarrow$} \\
    \cmidrule{1-11}
    %%% FINETUNER AVERAGE TASK = 9.29
    % FineTuner~\citep{yosinski2014transferable} && 78.1 (2.0) & 85.9 (2.3) && 63.1 (1.8) & 66.9 (2.4) && 4.01M & $(d_b + 1)C$ & \textbf{0.01M} \\

    % \cmidrule{1-11}
    % \metatune{} ProtoNets & N && \textbf{78.2 (1.9)} & 86.3 (2.2) && \textbf{65.7 (1.8)} & \textbf{70.7 (2.3)} && \textbf{4.01M} & $d_bC + |\vpsi|$ & 0.03M \\
    % \cmidrule{1-12}
    %%% SIMPLE CNAPs
    Simple CNAPs~\citep{bateni2020improved}  && 82.7 (1.7) & 91.8 (1.8) && 65.6 (1.9) & 71.9 (2.3) && 5.67M & $\frac{d_b(d_b + 3)}{2} C$ & 7.63M \\
    \cmidrule{1-11}
    %%% PROTONETS
    ProtoNets~\citep{snell2017prototypical} && 82.1 (1.7) & 91.2 (1.9) && 66.3 (1.8) & 72.9 (2.3) && \textbf{4.01M} & $d_bC$ & \textbf{0.01M} \\
    \cmidrule{1-11}
    %%% Ours
    \fit{}-LDA + ProtoNets~\citep{snell2017prototypical} && 82.9 (1.6) & 91.6 (1.8) && 66.7 (1.8) & 72.7 (2.3) && \textbf{4.01M} & $d_b \left(C + \frac{d_b + 1}{2}\right) + 2 + |\vpsi|$ & 0.85M \\
    % \cmidrule{1-11}
    %%%
    % \fit{}-LDA && 81.8 (1.8) & 90.6 (1.9) && 65.7 (1.8) & 70.7 (2.3) && \textbf{4.01M} & $d_b \left(C + \frac{d_b + 1}{2}\right) + 2 + |\vpsi|$ & 0.85M \\
    \bottomrule
    \end{tabular}}
    \vspace{0.5em}
\end{table}
